Boosting the 3D thermal-aware floorplanning problem through a master-worker parallel MOEA

The increasing transistor scale integration poses, among others, the thermal-aware floorplanning problem; consisting of how to place the hardware components in order to reduce overheating by dissipation. Due to the huge amount of feasible floorplans, most of the solutions found in the literature include an evolutionary algorithm for, either partially or completely, carrying out the task of floorplanning. Evolutionary algorithms usually have a bottleneck in the fitness evaluation. In the problem of thermal-aware floorplanning, the layout evaluation by the thermal model takes 99.5\% of the computational time for the best floorplanning algorithm proposed so far.The contribution of this paper is to present a parallelization of this evaluation phase in a master$-$worker model to achieve a dramatic speed-up of the thermal-aware floorplanning process. Exhaustive experimentation was done over three dimensional integrated circuits, with 48 and 128 cores, outperforming previous published works.

==> 04_conclusions.tex <==
\section{Conclusions}
\vspace{0.4cm}
Current and short term future state-of-the-art in 3D many-core integration requires thermal-aware floorplanning techniques able to reduce peak and mean temperatures. However, current techniques that take into account thermal issues spend the most of the execution time dealing with decodification and evaluation of solutions.

This work has proposed a parallel implementation of a thermal-aware Multi-objective Evolutionary Algorithm for 3D floorplanning using a master-worker scheme. This model has provided optimized configurations for systems composed of 48 and 128 heterogeneous processor cores.

We have shown that the highest speedup values are obtained when the number of workers is closer to the number of cores of the processor that runs the algorithm. In our experiments, run on a 4-core processor, we have obtained maximum speedup values of 3.79 and 3.19 respectively for the 48 and 128 core test configurations by selecting 5 workers in the optimization algorithm.

We have also shown that parallelization does not affect the quality of the solutions. Moreover, convergence evolves successfully in our experiments.

The parallelization of the algorithm has made possible the study of the convergence of our the proposed algorithm. The performed analysis has shown that convergence evolves successfully in our experiments.

% Working with thermally optimized heterogeneous architectures leads to a reduction of $66.52\,^{\circ}\mathrm{C}$ in the peak temperature of the chip with a minimum impact on performance.

Finally, we have proposed a new cell-based representation for the floorplanning solutions, more suitable for thermal simulators. This new representation will help obtaining more accurate thermal behavior of each individual, taking into account TSV. In addition, the grid-style of this new codification eases the parallelization through fine-grained approaches based, for instance, on GPUs. Our current work is focused on the study of this new representation, as well the parallelization of the MOEA using GPUs. 

==> 04_future.tex <==
\section{New Representation Proposal}

Once finished the study previously detailed, we aimed to overcome the drawbacks of the floorplan representation used in this work. Therefore, we propose a novel and simple representation suitable for fixed-outline floorplanning problems that allows a direct mapping of the individuals into configurations of the architecture. This is a major advantage and, with the use of this representation, the computational cost of the decoding step is avoided. Furthermore, it eliminates heuristics that might limit the exploration space and cause premature convergence problems.\\

As opposed to other representations such as Corner Sequence or O-tree, our new proposal is a non-compact representation that allows the use of \textit{free cells} as heat sinks to reduce the temperature of the chip. Free cells are \textit{free} in the sense that they do not contain functional units, but only wiring. Due to the lower temperature of wires in relation to functional units, these cells behave as coolers.

Also, this cell-level representation is in accordance with current thermal simulators such as 3D-ICE \cite{Sridhar2010} that split the IC into thermal cells. Therefore, the thermal error due to the different cell sizes used in the optimization and validation processes is eliminated. Thus, a better thermal optimization can be achieved.\\

In order to work with this representation, the IC is split into a mesh of cells. The choice of the cell size determines the granularity of the problem. In fact, considering big cells leads to a fast optimization process that may speedup the architectural exploration task. On the other hand, the smaller the cell size, the higher the accuracy of the thermal simulations is, but also the higher the complexity of the problem. In particular, floorplanning problems that consider the placement of Trough Silicon Vias (TSVs) are specially challenging as the pitch diameter of the TSVs is generally two orders of magnitude smaller than the components of the architecture. In order to deal with this increased difficulty, some proposals like \cite{Cuesta2011b} split the optimization process in two different steps performing the thermal optimization and the TSV placement in a sequential manner.

A different workaround is possible adopting a ``TSV-as-cell'' approach. The proposed representation is compatible with both strategies, and can minimize the area loss in the latter case considering a smaller cell size.\\

\begin{figure}[!h]
\centering
       \includegraphics[height=1.8in,width=3in]{fig/representation.png}
\caption{Configuration and representation of a simple architecture}
\label{representation}
\end{figure} 

Figure \ref{representation} shows a configuration and the corresponding representation of an architecture composed of 3 processors (C1, C2 and C3) and 3 memories (L1, L2 and L3). Each component of the architecture is characterized with a coordinate and a boolean flag. The coordinate determines the location of the left-bottom corner of the element while the flag indicates wether or not the given element is rotated. Therefore, the decodification of individuals is simpler than in the former representation of array of strings.

This grid-like representation admits a high level of parallelism and is well adapted for execution in massively parallel architectures such as GPUs. Nevertheless, appropriate operators need to be defined to ensure the generation of feasible solutions and the preservation of the diversity of the population.

A deeper study using this novel representation is our current and future work, and the preliminary results are very promising.

